SunStage: Portrait Reconstruction and Relighting using the Sun as a Light Stage

A light stage uses a series of calibrated cameras and lights to capture a subject's facial appearance under varying illumination and viewpoint. This captured information is crucial for facial reconstruction and relighting. Unfortunately, light stages are often inaccessible: they are expensive and require significant technical expertise for construction and operation. In this paper, we present SunStage: a lightweight alternative to a light stage that captures comparable data using only a smartphone camera and the sun. Our method only requires the user to capture a selfie video outdoors, rotating in place, and uses the varying angles between the sun and the face as guidance in joint reconstruction of facial geometry, reflectance, camera pose, and lighting parameters. Despite the in-the-wild un-calibrated setting, our approach is able to reconstruct detailed facial appearance and geometry, enabling compelling effects such as relighting, novel view synthesis, and reflectance editing. Results and interactive demos are available at https://sunstage.cs.washington.edu/.

==> fig_tex/data.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=.98\linewidth]{fig/data.pdf}
\end{center}
\caption{
% 
\textbf{Dataset -- }
}
\label{fig:dataset}
\end{figure}

==> fig_tex/perspective_ortho.tex <==
\begin{figure}
\begin{center}
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{fig/deca/1001_input.png}\\
\includegraphics[width=\linewidth]{fig/deca/1006_input.png}%
\caption{Input image}
\end{subfigure} \hfill %
\begin{subfigure}[b]{0.32\linewidth} %
\includegraphics[width=\linewidth]{fig/deca/1001_deca.png}\\
\includegraphics[width=\linewidth]{fig/deca/1006_deca.png}
\caption{Reconstructed model}
\end{subfigure} \hfill %
\begin{subfigure}[b]{0.32\linewidth}
\includegraphics[width=\linewidth]{fig/deca/1001_overlay.png}\\
\includegraphics[width=\linewidth]{fig/deca/1006_overlay.png}
\caption{Overlay}
\end{subfigure} 
\end{center}
\caption{
% 
\textbf{}
}
\label{fig:perspective}
\end{figure}

\vspace{-8mm}

==> fig_tex/results.tex <==
t\begin{figure*}
\begin{center}
\begin{subfigure}[b]{0.161\textwidth}
\includegraphics[width=\linewidth]{fig/applications/0043.png} %
\caption{Original}
\end{subfigure} \hfill %
\begin{subfigure}[b]{0.161\textwidth}
\includegraphics[width=\linewidth]{fig/applications/43_shadow.png} %
\caption{Reconstructed}
\end{subfigure} \hfill %
\begin{subfigure}[b]{0.161\textwidth} %
\includegraphics[width=\linewidth]{fig/applications/43_fill.png}
\caption{Added fill lighting}
\end{subfigure} \hfill %
\begin{subfigure}[b]{0.161\textwidth}
\includegraphics[width=\linewidth]{fig/applications/43_shadow_blurred_fill.png}
\caption{Fill + soft shadow}
\end{subfigure} \hfill %
\begin{subfigure}[b]{0.161\textwidth}
\includegraphics[width=\linewidth]{fig/applications/43_cayley_interior_2k.png}
\caption{Environment lighting}
\end{subfigure}
\begin{subfigure}[b]{0.161\textwidth}
\includegraphics[width=\linewidth]{fig/applications/43_chinese_garden_2k.png}
\caption{Environment lighting}
\end{subfigure}
\end{center}
\caption{
% 
\textbf{Applications -- }
Describe the above results.
}
\label{fig:overview}
\end{figure*}

==> fig_tex/teaser_6.tex <==
\begin{figure}
\captionsetup[subfigure]{justification=centering}
    \centering
\begin{subfigure}[t]{0.16\linewidth}
% \includegraphics[width=\linewidth]{fig/teaser/dan_input.png} %
% \end{subfigure}
% \begin{subfigure}[t]{0.16\linewidth}
% \includegraphics[width=\linewidth]{fig/teaser/dan_relight.png} %
% \end{subfigure}
% \begin{subfigure}[t]{0.16\linewidth}
% \includegraphics[width=\linewidth]{fig/teaser/dan_edit_albedo.png} %
% \end{subfigure}
% \begin{subfigure}[t]{0.16\linewidth}
% \includegraphics[width=\linewidth]{fig/teaser/dan_shiny.png} %
% \end{subfigure}
% \begin{subfigure}[t]{0.16\linewidth}
% \includegraphics[width=\linewidth]{fig/teaser/dan_envmap_inset.png} %

\includegraphics[width=\linewidth]{fig/teaser/florian_input.png} %
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/florian_relight_ns.png} %
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/florian_fillw.png} %
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/florian_env_inset_hair.png} %
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/florian_edit_albedo.png} %
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/florian_shiny.png} %
\end{subfigure}
\\
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/yifan_input.png} %
\caption{\\Reconstruction}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/yifan_relight_ns.png} %
\caption{\\Edit lighting}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/yifan_fillw.png} %
\caption{\\Soften shadows}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/yifan_env_inset_hair.png} %
\caption{\\Swap lighting}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/yifan_edit_albedo.png} %
\caption{\\Edit texture}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/teaser/yifan_shiny.png} %
\caption{\\Edit Materials}
\end{subfigure}
    \caption{\textbf{Our results}. Given a selfie video rotating under the sun, SunStage reconstructs geometry, material, camera pose, and lighting information. This recovered information can be used to (a) realistically re-render the input images, modify the lighting conditions by (b) adding / removing lights with different positions, sizes, and colors, or (c) changing existing light size to soften harsh shadows, (d) edit the albedo to add freckles, makeup, or stickers, (e) edit the material properties to increase or decrease shininess, or (f) render the person in an entirely new environment.}
    %edit the camera viewpoint or focal length.}
    \label{fig:teaser}

\vspace{-5mm}

\end{figure}
